T-GAP: Learning to Walk across Time for Temporal Knowledge Graph Completion

Temporal knowledge graphs (TKGs) inherently reflect the transient nature of real-world knowledge, as opposed to static knowledge graphs. Naturally, automatic TKG completion has drawn much research interests for a more realistic modeling of relational reasoning. However, most of the existing mod-els for TKG completion extend static KG embeddings that donot fully exploit TKG structure, thus lacking in 1) account-ing for temporally relevant events already residing in the lo-cal neighborhood of a query, and 2) path-based inference that facilitates multi-hop reasoning and better interpretability. In this paper, we propose T-GAP, a novel model for TKG completion that maximally utilizes both temporal information and graph structure in its encoder and decoder. T-GAP encodes query-specific substructure of TKG by focusing on the temporal displacement between each event and the query times-tamp, and performs path-based inference by propagating attention through the graph. Our empirical experiments demonstrate that T-GAP not only achieves superior performance against state-of-the-art baselines, but also competently generalizes to queries with unseen timestamps. Through extensive qualitative analyses, we also show that T-GAP enjoys from transparent interpretability, and follows human intuition in its reasoning process.

==> table/xyz_effect.tex <==
\begin{table}[htb] 
    \centering
    \small
    \begin{tabular}{ccc}
        \Xhline{2\arrayrulewidth}
        \multicolumn{1}{c|}{Configuration} & MRR & Inference Time \\
        \hline\hline
        \\[-1em]
        \multicolumn{1}{c|}{$x$: 5, $y$: 10, $z$: 10} & 0.599 & 539s \\
        \multicolumn{1}{c|}{$x$: 10, $y$: 100, $z$: 100} & 0.604 & 629s \\
        \multicolumn{1}{c|}{$x$: 50, $y$: 200, $z$: 200} & 0.606 & 941s \\
        \multicolumn{1}{c|}{$x$: 100, $y$: 500, $z$: 500} & 0.610 & 1233s \\
        \Xhline{2\arrayrulewidth}
    \end{tabular}
    \caption{Effect of different subgraph hyperparameters in ICEWS14. Inference time has been measured as time taken for 1 epoch in the test set, using 1 Tesla V100 GPU.}
    \label{tab:xyz_effect}
\end{table}
